Motion Planning for Robotics: A Review for Sampling-based Planners

Recent advancements in robotics have transformed industries such as manufacturing, logistics, surgery, and planetary exploration. A key challenge is developing efficient motion planning algorithms that allow robots to navigate complex environments while avoiding collisions and optimizing metrics like path length, sweep area, execution time, and energy consumption. Among the available algorithms, sampling-based methods have gained the most traction in both research and industry due to their ability to handle complex environments, explore free space, and offer probabilistic completeness along with other formal guarantees. Despite their widespread application, significant challenges still remain. To advance future planning algorithms, it is essential to review the current state-of-the-art solutions and their limitations. In this context, this work aims to shed light on these challenges and assess the development and applicability of sampling-based methods. Furthermore, we aim to provide an in-depth analysis of the design and evaluation of ten of the most popular planners across various scenarios. Our findings highlight the strides made in sampling-based methods while underscoring persistent challenges. This work offers an overview of the important ongoing research in robotic motion planning.

==> sections/sec7_something.tex <==
\begin{table}[H]
% \scriptsize % 缩小字体
\centering
\renewcommand{\arraystretch}{1.2} % Adjust row height
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{>{\centering\arraybackslash}p{3cm} >{\centering\arraybackslash}p{1cm} >{\centering\arraybackslash}p{3cm} >{\centering\arraybackslash}p{2.3cm} >{\centering\arraybackslash}p{2.5cm} >{\centering\arraybackslash}p{2cm} >{\centering\arraybackslash}p{2cm} >{\centering\arraybackslash}p{2cm} >{\centering\arraybackslash}p{2cm} >{\centering\arraybackslash}p{2cm} >{\centering\arraybackslash}p{2cm} >{\centering\arraybackslash}p{2cm} >{\centering\arraybackslash}p{2cm}}
\hline
% \begin{tabular}{p{2.5cm}p{1cm}p{3cm}p{2.3cm}p{2.5cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
\hline
\textbf{Method} & \textbf{Year} & \textbf{Probabilistic Completeness} & \textbf{Bidirectional Approach} & \textbf{Heuristic Implementation} & \textbf{Batch Sampling} & \textbf{Informed Search} & \textbf{Anytime} & \textbf{Lazy Evaluation} & \textbf{Greedy Strategy} & \textbf{learning-based} & \textbf{Static Path Planning} & \textbf{Dynamic Path Planning} \\
\hline
RRT~\cite{lavalle1998rapidly} & 1998 & \checkmark &  &  &  &  &  &  &  &  & \checkmark &  \\

RRT-connect~\cite{Kuffner2000rrt} & 2000 & \checkmark & \checkmark  &  &  &  &  &  &  &  & \checkmark &  \\

Lazy PRM~\cite{Bohlin2000path} & 2000 & \checkmark &  & \checkmark &  & \checkmark &  & \checkmark &  &  & \checkmark & \checkmark \\

hRRT~\cite{urmson2003approaches} & 2003 & \checkmark &  & \checkmark &  &  &  &  &  &  & \checkmark &  \\

ADD-RRT~\cite{Jaillet2005adaptive} & 2005 & \checkmark &  & \checkmark &  &  &  &  &  &  & \checkmark &  \\

Anytime RRT~\cite{Ferguson2006anytime} & 2006 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark \\

T-RRT~\cite{Jaillet2008transition} & 2008 & \checkmark &  & \checkmark &  &  &  &  &  &  & \checkmark & \checkmark \\

TSRRT~\cite{um2010tangent} & 2010 & \checkmark &  & \checkmark &  & \checkmark &  & \checkmark &  &  & \checkmark & \checkmark \\

RRT*~\cite{Karaman2011sampling} & 2011 & \checkmark &  & \checkmark &  &  & \checkmark &  &  &  & \checkmark &  \\

RRT*-SMART~\cite{Nasir2013RRT*-SMART} & 2013 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark &  \\

{RRT}$^\#$~\cite{arslan2013use} & 2013 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark \\

Informed RRT*~\cite{Gammell2014informed} & 2014 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark &  \\

FMT*~\cite{janson2015fastmarchingtreefast} & 2015 & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  & \checkmark & \\

BIT*~\cite{gammell2015batch} & 2015 & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  & \checkmark &  \\

Lazy-PRM*~\cite{hauser2015lazy} & 2015 & \checkmark &  & \checkmark &  & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark \\

Lazy-RRG*~\cite{hauser2015lazy} & 2015 & \checkmark &  & \checkmark &  & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark \\

RT-RRT*~\cite{naderi2015rt} & 2015 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark \\

B{I$^2$}RRT*~\cite{burget2016bi}  & 2016 & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark &  & \checkmark &  & \checkmark & \\

RR{T$^X$}~\cite{Otte2016rrtx} & 2016 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark \\

FCRRT~\cite{kang2016fast} & 2016 & \checkmark &  & \checkmark &  & \checkmark &  & \checkmark &  &  & \checkmark & \checkmark \\

HARRT*~\cite{Yi2016homotopy} & 2016 & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark \\

P-RRT*~\cite{Qureshi2016potential} & 2016 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark &  \\

ALCC~\cite{kim2018adaptive} & 2018 & \checkmark &  & \checkmark &  & \checkmark & \checkmark & \checkmark &  &  & \checkmark & \checkmark \\

NoD-RRT~\cite{Li2018neural} & 2018 & \checkmark & & \checkmark &  & \checkmark & \checkmark &  &  & \checkmark & \checkmark &  \\

PB-RRT*~\cite{tahir2018potentially} & 2018 & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark &  \\

PIB-RRT*~\cite{tahir2018potentially} & 2018 & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark &  \\

Multi-Tree T-RRT*~\cite{wong2018optimal} & 2018 & \checkmark &  & \checkmark &  & \checkmark &  &  &  &  & \checkmark & \checkmark \\

Lazy Steering RRT*~\cite{yavari2019lazy} & 2019 & \checkmark &  & \checkmark &  & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark &  \\

RL-RRT~\cite{chiang2019rl} & 2019 & \checkmark &  & \checkmark &  & \checkmark &  &  &  & \checkmark & \checkmark &  \\

Quick-RRT*~\cite{jeong2019quick} & 2019 & \checkmark &  & \checkmark &  &  & \checkmark &  &  &  & \checkmark &  \\

PQ-RRT*~\cite{li2020pq} & 2020 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark &  \\


AIT*~\cite{strub2020adaptively} & 2020 & \checkmark & \checkmark & \checkmark & \checkmark  & \checkmark & \checkmark &  &  &  & \checkmark & \\

ABIT*~\cite{strub2020advanced} & 2020 & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  & \checkmark &  \\

dRRT*~\cite{shome2020drrt} & 2020 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark \\



Neural RRT*~\cite{Wang2020neural} & 2020 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  & \checkmark & \checkmark &  \\

GBIT*~\cite{chen2021greedy} & 2021 & \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark &  & \checkmark &  \\

{MP-RRT}$^\#$~\cite{Primatesta2021amodel} & 2021 & \checkmark &  & \checkmark &  &  & \checkmark &  &  &  & \checkmark & \checkmark \\

AM-RRT*~\cite{Armstrong2021amrrt} & 2021 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark \\

MOD-RRT*~\cite{Qi2021mod} & 2021 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark \\

F-RRT*~\cite{Liao2021f} & 2021 & \checkmark &  & \checkmark &  &  & \checkmark &  &  &  & \checkmark & \checkmark \\

EIT*~\cite{strub2022adaptively} & 2022 & \checkmark &\checkmark  & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  & \checkmark & \\

EIRM*~\cite{hartmann2022effort} & 2022 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  & \checkmark & \\

RJ-RRT~\cite{chai2022rj} & 2022 & \checkmark &  & \checkmark &  & \checkmark &  &  & \checkmark &  & \checkmark & \\

BiAIT*~\cite{Li2023biait} & 2023 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  & \checkmark &  \\

EP-RRT*~\cite{ding2023improved} & 2023 & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark &  & \checkmark &  & \checkmark &  \\

FA-RRT*N~\cite{Khattab2023intelligent} & 2023 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark &  \\

GMM-RRT*~\cite{Lv2023gmm} & 2023 & \checkmark &  & \checkmark &  &  & \checkmark &  &  &  & \checkmark & \\

PROTAMP-RRT~\cite{saccuti2023protamp} & 2023 & \checkmark &  & \checkmark &  & \checkmark &  &  &  &  & \checkmark & \\

Neural Informed RRT*~\cite{huang2024neural} & 2024 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  & \checkmark & \checkmark & \checkmark \\

iDb-RRT~\cite{ortizharo2024idbrrt} & 2024 & \checkmark & \checkmark & \checkmark &  &  &  &  &  &  & \checkmark &  \\

SI-RRT*~\cite{sim2024safe} & 2024 & \checkmark &  & \checkmark &  & \checkmark & \checkmark &  &  &  & \checkmark & \checkmark \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of various sampling-based methods}
\end{table}
